Modular energy inequalities from relative entropy

We obtain new constraints for the modular energy of general states by using the monotonicity property of relative entropy. In some cases, modular energy can be related to the energy density of states and these constraints lead to interesting relations between energy and entropy. In particular, we derive new quantum energy inequalities that improve some previous bounds for the energy density of states in a conformal field theory. Additionally, the inequalities derived in this manner also lead us to conclude that the entropy of the state further restricts the possible amount of negative energy allowed by the theory.

==> Changes <==
----- pst-tree.tex
1.11  2009-09-17 - fix bug with bounding box 
1.10  2009-01-25 - first version with pst-xkey and own 
                   documentation (hv) 
1.01  2007-01-03 - fix bug with \endpsTree (hv) 


----- pst-tree.sty
     2008-12-12 first version (hv) 



==> Settings.tex <==
%paquetes


\usepackage{amsmath}
\DeclareMathOperator\arctanh{arctanh} % Arctan(x)
\newcommand{\normord}[1]{:\mathrel{#1}:} %Orden normal
\usepackage{amssymb}
\usepackage{braket} %Para utilizar notacion de bracket de Dirac
%\usepackage{xr} %Para hacer referencias entre distintos .tex archivos

\usepackage{graphicx}
\usepackage[spanish]{babel} % option es-lcroman para numeros romanos en minuscula
\usepackage[utf8]{inputenc}
\usepackage{textcomp}
\usepackage{float}
\usepackage[labelfont=bf, textfont=normal,
			justification=justified,
			singlelinecheck=false]{caption}
\usepackage[labelfont=bf, textfont=normal,
			justification=justified,
			singlelinecheck=false]{subcaption}
\usepackage{multirow}
\usepackage{amsmath}
%\usepackage{subfig}
%\usepackage[retainorgcmds]{IEEEtrantools} %% Esto es para insertar links a páginas web.
\usepackage{multicol}
\usepackage[table]{xcolor} %para pintar celdas con el comando \cellcolor{red}
\usepackage{hyperref} % para poner liks dentro y fuera del documento con el comando \href{<my_url>}{<description>}. Buscar mas funcionalidades.
\hypersetup{colorlinks, citecolor=black,
   		 	filecolor=black, linkcolor=black,
    		urlcolor=black}
% \usepackage[version=4]{mhchem} % Para graficar reacciones químicas

%agregar notas al pdf
\usepackage[textsize=footnotesize,backgroundcolor=green!40]{todonotes}
\presetkeys{todonotes}{inline}{}

% Lenguajes de Programacion
%\usepackage[]{mcode} % paquete para agregar código de MatLab. Es necesario copiar el mcode.sty https://www.sharelatex.com/project/5539017293616a9c19e2cd24
%\usepackage{listings} %para incluir varios lenguajes de programacion (Ej: Python)

% Caracteristicas de paginas

\usepackage[top=3cm, bottom=3cm,
			inner=2cm, outer=1.5cm]{geometry}			% Page margin lengths

%\pdfpagewidth 8.5in
%\pdfpageheight 11in
%\setlength\oddsidemargin{-0,21in}
%\setlength\evensidemargin{-0,21in}
%\setlength\topmargin{-2cm}
%\setlength\textwidth{7in}
%\setlength\textheight{23.7cm}
\setlength\parskip{0.1in}


% Caracteristicas de estilo

%\usepackage{setspace}
%\onehalfspacing

% Cambiar nombre de tablas

\renewcommand{\listtablename}{Indice de tablas}
	\renewcommand{\tablename}{Tabla}


% Formato de los títulos de capítulos
\usepackage{titlesec}		
\titleformat{\chapter}[display]
  {\Huge\bfseries\filcenter}
  {{\fontsize{50pt}{1em}\vspace{-4.2ex}\selectfont \textnormal{\thechapter}}}{1ex}{}[]





% Defino Funciones comunes

\newcommand{\ening}[1]{\textit{#1}}
